Can Pairwise Testing Perform Comparably to Manually Handcrafted Testing Carried Out by Industrial Engineers?

Testing is an important activity in engineering of industrial software. For such software, testing is usually performed manually by handcrafting test suites based on specific design techniques and domain-specific experience. To support developers in testing, different approaches for producing good test suites have been proposed. In the last couple of years combinatorial testing has been explored with the goal of automatically combining the input values of the software based on a certain strategy. Pairwise testing is a combinatorial technique used to generate test suites by varying the values of each pair of input parameters to a system until all possible combinations of those parameters are created. There is some evidence suggesting that these kinds of techniques are efficient and relatively good at detecting software faults. Unfortunately, there is little experimental evidence on the comparison of these combinatorial testing techniques with, what is perceived as, rigorous manually handcrafted testing. In this study we compare pairwise test suites with test suites created manually by engineers for 45 industrial programs. The test suites were evaluated in terms of fault detection, code coverage and number of tests. The results of this study show that pairwise testing, while useful for achieving high code coverage and fault detection for the majority of the programs, is almost as effective in terms of fault detection as manual testing. The results also suggest that pairwise testing is just as good as manual testing at fault detection for 64% of the programs.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tables/statisticComparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.5}
\caption[Statistical Analysis of the results]{Statistical analysis of the results presented after evaluating the strength of the pairwise and manual approach to the random one.} 
\resizebox{\columnwidth}{!}{ %resize the table to fit in the column.
\begin{tabular}{l|l|r|r|}
\cline{2-4}
Statistics & Values & \multicolumn{1}{l|}{Code Coverage}	 & \multicolumn{1}{l|}{Mutation Score} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{$S_{P} - S_{R}$}}    	& $\vcenter{\hbox{$\hat{A}$}}$ 	& 0.69                                 & 0.55\\ \cline{2-4} 
\multicolumn{1}{|l|}{}                  					& $p-value$ 					& $<$0.01                              & 0.40\\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{$S_{E} - S_{R}$}}    	& $\vcenter{\hbox{$\hat{A}$}}$ 	& 0.78                                 & 0.58\\ \cline{2-4} 
\multicolumn{1}{|l|}{}                  					& $p-value$ 					& $<$0.01                              & 0.17\\ \hline
\end{tabular}





% \begin{tabular}{l|l|r|r|r|}
% \cline{2-5}
% Statistics & Values & \multicolumn{1}{l|}{Code Coverage} & \multicolumn{1}{l|}{Mutation Score} & \multicolumn{1}{l|}{Test Suite Size} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{$S_{P} - S_{R}$}}    & $\vcenter{\hbox{$\hat{A}$}}$ & 0.69                                 & 0.55                               & -                               \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                  				& $p-value$ 	& $<$0.01                                & 0.40                           & -                            \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{$S_{E} - S_{R}$}}    & $\vcenter{\hbox{$\hat{A}$}}$ & 0.78                                 & 0.58                               & -%0.53
% \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                  				& $p-value$ 	& $<$0.01                                 & 0.17                           & -%0.64
% \\ \hline
% \end{tabular}








% \begin{tabular}{l|l|r|r|r|}
% \cline{2-5}
% Statistics & Values & \multicolumn{1}{l|}{$S_{M} - S_{P}$} & \multicolumn{1}{l|}{$S_{P} - S_{R}$} & \multicolumn{1}{l|}{$S_{M} - S_{R}$} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{Code Coverage}}    & $\vcenter{\hbox{$\hat{A}$}}$ & 0.60                                 & 0.69                              & 0.78                               \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                  				& p-value 	& 0.04                                 & $<$0.01                           & $<$0.01                            \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{Mutation Score}}   & $\vcenter{\hbox{$\hat{A}$}}$ & 0.53                                 & 0.55                              & 0.58                               \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                                  & p-value 	& 0.67                                 & 0.40                              & 0.17                            \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{Test Suite Size}}	& $\vcenter{\hbox{$\hat{A}$}}$ & 0.53                                 & -                                 & 0.53                               \\ \cline{2-5} 
% \multicolumn{1}{|l|}{}                               	& p-value	& 0.64                                 & -                                 & 0.64                               \\ \hline
% \end{tabular}
}
%\vspace*{0.5cm}
%\vspace*{0.5cm}
\label{table:statisticalComparison}
\end{table}

